Comparison of Microservice Call Rate Predictions for Replication in the Cloud

Today, many users deploy their microservice-based applications with various interconnections on a cluster of Cloud machines, subject to stochastic changes due to dynamic user requirements. To address this problem, we compare three machine learning (ML) models for predicting the microservice call rates based on the microservice times and aiming at estimating the scalability requirements. We apply the linear regression (LR), multilayer perception (MLP), and gradient boosting regression (GBR) models on the Alibaba microservice traces. The prediction results reveal that the LR model reaches a lower training time than the GBR and MLP models. However, the GBR reduces the mean absolute error and the mean absolute percentage error compared to LR and MLP models. Moreover, the prediction results show that the required number of replicas for each microservice by the gradient boosting model is close to the actual test data without any prediction.

==> Figures/old/old-text.tex <==

% \subsection{Prediction model}
% We define a linear regression prediction model for microservice call rate prediction, aiming at a minimum error between the predicted microservice call rate and the actual one.
% \subsubsection{Linear regression} defines a relation between the $\mt\left(m_i,\DATA_{ui},r_j\right)$ and the microservice call rate $\mcr_{ui}$. We define the scheduling of microservice $m_i$ on a resource $r_j = \sched(m_i)$. Thereafter, we model a linear relation between microservice call rate $\mcr_{ui}$ and microservice time $\mt=\{\mt\left(m_i,\DATA_{ui},r_j\right)|\ r_j = \sched(m_i)\}$ according to a set of weights $\w =\{\w\left(m_i,\DATA_{ui}, r_j\right)|0\le i<\mathcal{N}_{\mathcal{M}}\}$ and a constant $\epsilon$:
% \begin{equation*}
%     \mcr^{\prime} = \sum\limits_{\substack{m_i\in\mathcal{M}\land \\ r_j = \sched(m_i)}} \{\mt\left(m_i,\DATA_{ui},r_j\right)\cdot \w\left(m_i,\DATA_{ui}, r_j\right)+\epsilon\},
% \end{equation*}
% where $\w\left(m_i,\DATA_{ui},r_j\right)$ is the weight of a microservice time $\mt\left(m_i,\DATA_{ui},r_j\right)$.
% %A linear relation between output variable Y and input variables $X= x_1 x_n$, and attempts to find a vector $\beta =\{w_1,\cdot, w_n\}$  and a scalar b where Y = XW+b with the goal of minimizing the error = $|Y-Y^{\prime}|$. Minimization is usually performed using the least square error~\cite{iqbal2019adaptive}.


Figures~\ref{fig:pred-lr}, \ref{fig:pred-mlp}, and \ref{fig:pred-gbr} show the prediction models' performance over the test data. In row number \num{1200} of the test data, the GBR method predicts with higher accuracy compared to the two other methods.
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/lr-predict.png}
%     \caption{Comparison of the actual and predicted MCR of the linear regression model.}
%     \label{fig:pred-lr}
% \end{figure}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/mlp-predict.png}
%     \caption{Comparison of the actual and predicted MCR of the multilayer perceptron model.}
%     \label{fig:pred-mlp}
% \end{figure}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/gbr-predict.png}
%     \caption{Comparison of the actual and predicted MCR of the gradient boosting regression model.}
%     \label{fig:pred-gbr}
% \end{figure}
